Artificial Intelligence for Digital Agriculture at Scale: Techniques, Policies, and Challenges

Digital agriculture has the promise to transform agricultural throughput. It can do this by applying data science and engineering for mapping input factors to crop throughput, while bounding the available resources. In addition, as the data volumes and varieties increase with the increase in sensor deployment in agricultural fields, data engineering techniques will also be instrumental in collection of distributed data as well as distributed processing of the data. These have to be done such that the latency requirements of the end users and applications are satisfied. Understanding how farm technology and big data can improve farm productivity can significantly increase the world's food production by 2050 in the face of constrained arable land and with the water levels receding. While much has been written about digital agriculture's potential, little is known about the economic costs and benefits of these emergent systems. In particular, the on-farm decision making processes, both in terms of adoption and optimal implementation, have not been adequately addressed. For example, if some algorithm needs data from multiple data owners to be pooled together, that raises the question of data ownership. This paper is the first one to bring together the important questions that will guide the end-to-end pipeline for the evolution of a new generation of digital agricultural solutions, driving the next revolution in agriculture and sustainability under one umbrella.

==> Team.tex <==
\textbf{Rationale}
Dr. Chaterji works in the areas of data science and engineering for digital agriculture and genomics and in building cyberinfrastructures for these domains. She is a part of the WHIN (Wabash Heartland Innovation Network) leadership team working to bring IoT to advance agriculture. Data is power! She believes in leveraging the power of big data by drawing actionable insights from diverse agricultural sensing data to make agricultural practices high-throughput and sustainable. As a second thrust of her work, Dr. Chaterji is extracting insights from epigenomic data for predictive and personalized healthcare, one in which health and vitality is the focus. To accomplish her goals, Dr. Chaterji develops algorithms and statistical models for precision medicine, and more recently, in digital agriculture with an eye toward sustainability.

Dr. DeLay’s research focuses on the decision making processes of commercial producers. Using producer level and aggregated longitudinal data, he has estimated the impact of government policies on land use and production decisions, exploiting various econometric techniques to identify causal relationships. Dr. DeLay was hired in the Fall of 2018 to contribute to the College of Agriculture’s focus on digital agriculture where he is studying the impact of data use and technology adoption on measures of productivity. He is currently designing a comprehensive producer survey to understand the value of farm data collected by commercial operators and how this value is channeled in the production process. 

==> perspectives.tex <==
\section{Future Perspectives}

This article highlights the challenges in bringing the benefits of
AI and ML to agriculture, and presents a few promising solutions. These technologies will become even more pervasive with the advent of a few key technologies. 

With Edge computing, computing moves closer to the data collection devices, such as sensors, drones, cameras, and tractors. Cameras could detect weeds, drones could detect stress in flight, and only transmit images that have stress.  

==> proposal.tex <==
\section{Proposal}
\thispagestyle{plain}
%\vspace{-20pt}
\begin{itemize}
 \addtolength\leftmargin{-3em}
  \item {\bf Target journal}: Communications of the ACM (CACM). IF = 3.063. This is the premier, common interest magazine in the Computer Science field and our paper fits in the ``Contributed Article'' category.   
  \item {\bf Author list}: Somali Chaterji (Agricultural and Biological Engineering, ABE), John Evans (ABE), Nathan DeLay (Agricultural Economics), Nathan Mosier (Indiana Soybean Board Professor), Dennis Buckmaster (Dean's Fellow, ABE) (Purdue University); Ranveer Chandra (Chief Scientist, Microsoft Azure Global). The  team  comprises of experts  in  digital  agriculture, applied 
 data  analytics, and  agricultural  policy on the academic side, together with a leading exponent of cloud computing in agriculture from the private sector. This paper builds on existing expertise and publications of the team members, namely, Chaterji in applied data analytics and data engineering~\cite{koo2018tiresias, kim2016opening, ghoshal2015microrna, ghoshalTCGA, mahgoub2017rafiki, wilke2015mg}, Evans in agricultural sensing~\cite{sama2016applied, evans2017automated}, DeLay in agricultural policy~\cite{delay-1, delay-2}, Buckmaster in farm information systems and data flow~\cite{noel2018real, wang2016candroid, balmos2016investigation, buckmaster2016digital, buckmaster2018precision}, Mosier in sustainable agriculture~\cite{parsell2015synergistic, abu2017atomic}, and Chandra in networking and sensors~\cite{bahl2009white, chandra2007location, saifullah2016snow}. Chandra also has prior experience of publishing in CACM. Therefore, our team is  uniquely  qualified  to  write  this  article,  which will hopefully energize the community to search for answers in data analytics for sustainable and digitized agriculture.
  \item {\bf Paper goals}: There  are  important  questions  to  be  answered  before  we  can  leap  into  data  analytics  for  agriculture,  questions  related  to technical viability, economic feasibility, and data protection and ownership. These questions cannot be looked at in isolation---for  example,  if  some  algorithm  needs  data  from  multiple  data  owners  to  be  pooled  together,  that  raises  the  question  of  data ownership.  This  paper  is  the  first  to  bring  together  these  questions  under  one  umbrella.
  \item {\bf Paper significance}: By 2050, the world's population will increase to nine billion, which will aggravate the food-water-energy nexus challenges. Demand will also rise because of increase in people's wealth resulting in higher meat consumption plus the increasing use of cropland for biofuels. Site-specific farm management (precision farming) has the potential to nourish the world while increasing farm profitability under constrained resource conditions. Despite advancements in field sensors, GPS, and grid soil sampling, adoption of technology by farm operators has fallen short of expectations~\cite{schimmelpfennig2016farm, bullock2009value, baerenklau2007dynamics}. Moreover, it is unclear how profitable the adoption of such technologies will be~\cite{bullock2000agronomic}.
Operator demographics, operation size, and perceived benefits influence the decision to invest in site-specific management practices and adoption rates vary widely across technology types~\cite{thompson2019farmer, schimmelpfennig2016farm}. Use of variable rate technology (VRT), for example, has lagged that of yield monitors and automated guidance systems. An important distinction has been drawn between farm technology and the farm information that complements the technology~\cite{bullock2009value}. For example, the economic benefit of a variable rate fertilizer depends on accurate intra-field soil data, which is itself expensive to obtain. Unless the economic returns to site-specific management cover both the up-front investment and the cost of collecting quality information, adoption will be low. 
The topic of digital agriculture, encompassing precision (data-driven) agriculture, data analytics, and data ownership, is  an  important  focus  area  for  the  College  of  Agriculture  and  the  Departments of   Agricultural  and  Biological  Engineering (ABE) \textit{and}  Agricultural Economics. The College can fulfill the land grant mission in the 21st century by understanding  how  farm  technology  and  big  data  can  improve  farm  productivity and that too under constrained resources.  While  much  has  been  written  about  digital agriculture's potential, little is known about the economic costs and benefits of these emergent systems. In particular, the on-farm decision making processes, both in terms of adoption and optimal implementation, have not been adequately addressed. This paper raises important questions and surveys some leading edge tools and techniques from computational science and engineering that can be harnessed for this area and the policy guidelines that will need to be taken into consideration while deploying the farm-management sensors and algorithms. 
\end{itemize}

\subsection*{\textbf{Paper outline}}
\bigskip
\noindent \url{https://docs.google.com/document/d/1xVQmJ8DLSZOB7-jF8yiHQ0_wbryBj_vH3_9CalDelXU/edit}

This paper looks at the lifecycle of big data techniques applied to agricultural data as related to the evolution of precision or data-driven agriculture. It starts from the data origination by a profusion of sensors (ground sensors, aerial sensors, etc.), which monitor physical, biological, and chemical phenomena to generate data elements, then considers the data hygiene and data preprocessing required to integrate the different modalities of sensing for amplified and more accurate sensing, leading to ML technologies invoked through popular big data frameworks. The paper then gets into the policy questions surrounding the use of big-data technologies. For each part, we survey what is the current state-of-practice and then provide the most important open questions. 

{\color{blue}{\noindent [Participants for individual bullet points in blue, lead for the bullet point in \textbf{bold} blue.]}}
\begin{enumerate}

   \item {\em Data generation and flow from in-ground, machine, and drone-based sensors}. This will cover the modalities of data gathering and controlled dissemination, the volume of data generated, and the quality of the data. {\color{blue} [Participants: Evans, \textbf{Buckmaster}, Chandra]}

   \item {\em Data life cycle}. This will cover the various phases in the lifecycle of big agricultural data---sanitization, loading, processing, storing, summarization, and analysis. This will go into some of the general-purpose approaches (such as, data deduplication, calibration using sensor metadata) as well as agricultural-specific approaches (such as, known variations in hyperspectral maps from ground sensing and aerial image data and effective fusion among sensor arrays). {\color{blue} [Participants: \textbf{Evans}, Buckmaster]} 

   \item {\em Machine learning technologies}. This will cover approximate processing for in-sensor analytics, advanced processing for backend analytics on the edge or the cloud platforms, and interpretable data analytics. The first aspect is particularly useful because of the expensive nature of the wireless communication or the lack of continuous connectivity of the sensors to the backend. The second aspect is useful because there are edge platforms for agricultural data, such as, Azure IoT Edge device, and there may be sensitivity of the farmer to upload her personal data to a cloud platform. The final aspect is important because the farmer, a non-data science expert, will still need to be given some insights into the results of the algorithm, at her level of understanding, before such a person will take actionable measures.  {\color{blue} [Participants: \textbf{Chaterji}, Chandra]} 
   
   %\item {\em FarmBeats and AirBand
   \item \textit{Democratizing Artificial Intelligence (AI) for farmers.} This will cover some of the foundational technologies that can result in farms---even small-scale farms---deploying leading-edge AI tools and broadband modalities to gather data from farms (e.g., FarmBeats, AirBand technologies, Open Ag Data Alliance APIs). This will cover the commercial angle of deploying and operating a system and the foundational (and often open-source) technologies that they build upon, such as, TV whitespace spectrum being used to upload high volume data. {\color{blue} [Participants: \textbf{Chandra}, Chaterji]} 

   \item {\em Big data frameworks for agricultural data}. Here we will discuss the popular frameworks through which we will invoke the machine learning (ML) algorithms. This will involve open source frameworks such as Apache Spark, streaming data processing frameworks such as Apache Flink, and techniques for distributing the ML processing among nodes in a cluster. {\color{blue} [Participants: \textbf{Chaterji}, Chandra]} 
     
   \item {\em Big data in alternative farming}. We will develop the ideas of big data algorithms being used to optimize alternative farming practices, such as, biofuels. {\color{blue} [Participants: \textbf{Mosier}, Chaterji]} 
   
   \item {\em Policy issues}. We will discuss the policy issues that should regulate the use of big data and the economic factors that will be important for the adoption of big data. The most relevant policy questions in digital agriculture regard the value and legal status of farm and related business data. Though farm data enjoy some of the intellectual property protections afforded to trade secrets, its legal ownership structure remains ambiguous~\cite{miller2018estimating, ferrell2016legal}. The decision to subscribe to a data service provider may be impacted by fears of personally identifiable information (PII) being misappropriated. Yet farm data generates positive network externalities when aggregated across a large number of operations. Business models, such as Farmers Business Network, Inc. (FBN), have demonstrated the value of data sharing. Academic research should focus on designing incentive-compatible mechanisms that encourage data sharing with public universities while protecting farmers’ intellectual property (IP). {\color{blue} [Participants: \textbf{DeLay}, Chandra]} 
\item Future perspectives. {\color{blue} [Participants: Evans, DeLay, Chaterji, \textbf{Chandra}}]
\end{enumerate}

\subsection*{\textbf{Anticipated Research Opportunities}}

This paper would position our research team for the following initiatives:
\begin{itemize}
    \item Wabash Heartland Innovation Network (WHIN) and Lilly Foundation grants
    \item USDA NIFA Sustainable Agriculture Systems and AFRI Foundational and Applied Science
    \item NSF Cyber-Physical Systems (CPS)-USDA
\end{itemize}
The focus areas within the USDA grants that we would be positioned to address are: ``Agriculture Systems and Technology''  and ``Agriculture Economics and Rural Communities''. For AFRI, we will focus on Bioenergy and Agriculture Systems and Technology. Research-only, extension-only, and integrated research, education and/or extension projects are solicited in this Request for Applications (RFA). 

\vspace{2pt}
\noindent{This will also be the start of a productive collaboration between the FarmBeats project in Microsoft Azure and Purdue's Colleges of Agriculture and Engineering.} 
\newpage
\section*{Supporting Information and Bibliography}

\begin{enumerate}
    \item {\em Selection of the research issue and its strategic importance}: 
The research issue we are addressing is unique in that it aligns with three of the four themes for the ``150 Years of Giant Leaps'' program, namely, ``Artificial Intelligence (AI)'', ``Sustainability'', and ``Health and Longevity''. For AI, we will be discussing full-stack data science and engineering for the myriad agricultural sensing data and how to draw insights from them by using AI/ML techniques. For Sustainability, our discussion will shed light on how agricultural practices can be made more sustainable, i.e., do more with less (resources), using the large amounts of data that are already being generated. For Health and Longevity, we describe how food cannot just feed the burgeoning population, but also nourish it.
    
    \item {\em Rationale for the team of authors}: The team comprises researchers and practitioners with complementary skills and who have already started working together: Chaterji in applied data analytics, Evans in precision-agriculture sensors, Buckmaster in machine systems and digital agriculture, DeLay in agricultural economics, Mosier in alternative farming and sustainability, and Chandra from the private sector in a commercialization venture in digital agriculture. 
    
    \item {\em Specific funding opportunities}: We have already described some above. In addition, on the more foundational side, this paper will also elevate our stature for panelists in the NSF Computing Directorate (CISE) IIS program as well as the NIH's NIAID and NIGMS Institutes. 
 \item{Expected date of submission}: August 2019.    
\end{enumerate}
\vspace{-15pt}

\pagebreak
%\bibliographystyle{ieeetr}
%\bibliography{ref}

% SC (2/22/19): Commented out for the 2 page proposal


% Note that keywords are not normally used for peerreview papers.
%\begin{IEEEkeywords}

%\end{IEEEkeywords}

